Personalized advice for enhancing well-being using automated impulse response analysis --- AIRA

The attention for personalized mental health care is thriving. Research data specific to the individual, such as time series sensor data or data from intensive longitudinal studies, is relevant from a research perspective, as analyses on these data can reveal the heterogeneity among the participants and provide more precise and individualized results than with group-based methods. However, using this data for self-management and to help the individual to improve his or her mental health has proven to be challenging. The present work describes a novel approach to automatically generate personalized advice for the improvement of the well-being of individuals by using time series data from intensive longitudinal studies: Automated Impulse Response Analysis (AIRA). AIRA analyzes vector autoregression models of well-being by generating impulse response functions. These impulse response functions are used in simulations to determine which variables in the model have the largest influence on the other variables and thus on the well-being of the participant. The effects found can be used to support self-management. We demonstrate the practical usefulness of AIRA by performing analysis on longitudinal self-reported data about psychological variables. To evaluate its effectiveness and efficacy, we ran its algorithms on two data sets ($N=4$ and $N=5$), and discuss the results. Furthermore, we compare AIRA's output to the results of a previously published study and show that the results are comparable. By automating Impulse Response Function Analysis, AIRA fulfills the need for accurate individualized models of health outcomes at a low resource cost with the potential for upscaling.

==> output/tab_comparison_javascript.tex <==
% latex table generated in R 3.3.0 by xtable 1.8-2 package
% Sun May 15 11:50:00 2016
\begin{table}[ht]
\centering
\resizebox{\columnwidth}{!}{
\begin{tabular}{rrrrr}
  \toprule
 & Activity (\textsc{aira}) & Activity (vars) & Depression (\textsc{aira}) & Depression (vars) \\ 
  \midrule
  1 & 1.000 & 1.000 & 0.000 & 0.000 \\ 
  2 & 0.463 & 0.463 & -0.178 & -0.178 \\ 
  3 & 0.462 & 0.462 & -0.149 & -0.149 \\ 
  4 & 0.328 & 0.328 & -0.157 & -0.157 \\ 
  5 & 0.266 & 0.266 & -0.133 & -0.133 \\ 
  6 & 0.204 & 0.204 & -0.114 & -0.114 \\ 
  7 & 0.160 & 0.160 & -0.094 & -0.094 \\ 
  8 & 0.125 & 0.125 & -0.076 & -0.076 \\ 
  9 & 0.097 & 0.097 & -0.061 & -0.061 \\ 
  10 & 0.076 & 0.076 & -0.048 & -0.048 \\ 
   \bottomrule
\end{tabular}
}
\caption{Comparison between the outcomes of the JavaScript version of AIRA and the R package 'vars', using the model and data from the study by \citeauthor{RefWorks:4}} 
\label{tab:comparison_javascript}
\end{table}


==> output/tab_effects.tex <==
% latex table generated in R 3.3.1 by xtable 1.8-2 package
% Fri Sep 16 13:16:24 2016
\begin{table}[ht]
\centering
\resizebox{\columnwidth}{!}{
\begin{tabular}{rll}
  \toprule
 & Activity to improve Depression & Depression to improve Activity (\textsc{aira}) \\ 
  \midrule
pp1 & No effect & -253.3\% \\ 
  pp2 & 507.58\% & No effect \\ 
  pp4 & No effect & No effect \\ 
  pp5 & 10151.34\% & No effect \\ 
   \bottomrule
\end{tabular}
}
\caption{\citeauthor{RefWorks:4}~\cite{RefWorks:4}.} 
\label{tab:effects}
\end{table}


==> output/tab_percentage_effects_in_aira.tex <==
% latex table generated in R 3.3.1 by xtable 1.8-2 package
% Fri Sep 16 13:18:44 2016
\begin{table*}[ht]
\centering
\begin{tabular}{rllllll}
  \toprule
 & decrease feeling gloomy by changing relaxation & decrease feeling gloomy by changing feeling inadequate & increase relaxation by changing feeling gloomy & increase relaxation by changing feeling inadequate & decrease feeling inadequate by changing feeling gloomy & decrease feeling inadequate by changing relaxation \\ 
  \midrule
Person 1 & $\infty$ & $\infty$ & $\infty$ & $\infty$ & $\infty$ & $\infty$ \\ 
  Person 2 & $\infty$ & $\infty$ & $\infty$ & $\infty$ & -89.89\% & $\infty$ \\ 
  Person 3 & $\infty$ & $\infty$ & $\infty$ & 0\% & $\infty$ & $\infty$ \\ 
  Person 4 & $\infty$ & $\infty$ & $\infty$ & $\infty$ & $\infty$ & $\infty$ \\ 
  Person 5 & $\infty$ & $\infty$ & $\infty$ & $\infty$ & $\infty$ & 206.38\% \\ 
   \bottomrule
\end{tabular}
\caption{Effects of Feeling less gloom, inadequate and relaxation on well-being} 
\label{tab:percentage_effects_in_aira}
\end{table*}


==> output/tab_supported_functions.tex <==
% latex table generated in R 3.3.1 by xtable 1.8-2 package
% Fri Sep 16 13:18:44 2016
\begin{table}[ht]
\centering
\centering
\resizebox{\columnwidth}{!}{
\begin{tabular}{lll}
  \toprule
 & Aira js & Aira-R \\ 
  \midrule
DetermineOptimalNode & Yes & Yes \\ 
  DetermineLengthOfEffect & Yes & Yes \\ 
  DeterminePercentageEffect & Yes & Yes \\ 
  Impulse Response Function Analysis & Yes & Yes \\ 
  Animations and Visual representation & Yes & No \\ 
  Interactivity & Yes & No \\ 
  Orthogonalized Impulse Response Function Analysis & No & Yes \\ 
  Bootstrapping & No & Yes \\ 
   \bottomrule
\end{tabular}
}
\caption{Supported functions of both implementations of AIRA} 
\label{tab:supported_functions}
\end{table}

